Fluid deformable surfaces with variable thickness - a Surface Shallow-Water-Helfrich model

Epithelial tissues play a fundamental role in morphogenesis. Mechanically they can be viewed as thin soft materials exhibiting a solid-fluid duality. The Surface Navier-Stokes-Helfrich model accounts for these properties by combining bending and surface hydrodynamics. In order to account for varying cell thickness we incorporate a thickness field in the spirit of a shallow-water equation, but defined on the (self-)evolving surface. This replaces the inextensibility constraint of the two-dimensional fluid and with it the conservation of surface area by an incompressibility constraint of the thin film fluid allowing for changes in surface area. We develop a numerical scheme based on surface finite elements, perform convergence tests, demonstrate the impact on shape evolution of closed surfaces with a constant enclosed volume and discuss implications on modeling morphogenesis.

==> newcommands.tex <==
\usepackage{mathrsfs}
\usepackage{scalerel}

\DeclareMathAlphabet{\Mymathbb}{U}{bbold}{m}{n}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}
% \DeclareMathOperator*{\dprime}{\prime \prime}
%==========================================================================
% % % %                      NEW COMMANDS                         % % % % % 
%==========================================================================

\newcommand{\Reylightian}{\mathcal{R}}


\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}


\newtheorem{remark}{Remark}
\newtheorem{problem}{Problem}
\newtheorem{example}{Example}



%======================================================
\newcommand{\T}{\mbox{\tiny T}}
\newcommand{\disp}{\mbox{\tiny disp}}
\newcommand{\Forall}{\forall \,}%{\mbox{ for all }}


\newcommand{\timeSymbol}{t}
\newcommand{\Time}{\timeSymbol} %generic time
\newcommand{\TimeF}{T} %final time
\newcommand{\tempo}{\Time} %generic time
\newcommand{\Tempo}{\TimeF} %final time

%======================================================
% volume form
\newcommand{\VolForm}{\Diff V_{\First}}

% Metric Tensor - Fundamental forms
\newcommand{\FirstSymbol}{\mathcal{G}}
\newcommand{\First}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\FirstSymbol}
  {\FirstSymbol_{\scriptscriptstyle{#1}}}
}
\newcommand{\EigFirst}{{\mu_{\scriptscriptstyle{\First}}}}
\newcommand{\EigFirstInvmin}{g_{*}}
\newcommand{\EigFirstInvmax}{g^*}
\newcommand{\CminDetG}{c_{\scriptscriptstyle{\First}}}
\newcommand{\CmaxDetG}{C_{\scriptscriptstyle{\First}}}
\newcommand{\ConstGeom}[1][]{
   \ifthenelse{\equal{#1}{}}       
   {K_{\First}\,}
   {K_{\First,#1}\,}
}

\newcommand{\FirstForm}[1][]{
  \ifthenelse{\equal{#1}{}}       
  {\operatorname{I_{\point}}}             
  {\operatorname{I_{#1}}}             
}
%=================== operators ========================
\newcommand{\GradSymbol}{\operatorname{\mathbf{\nabla}}}
\newcommand{\Grad}{\GradSymbol}
\newcommand{\Div}{\Grad\cdot}
\newcommand{\Lap}{\Delta}

\newcommand{\GradSurf}{\GradSymbol_{\!\SurfDomain}\!}
\newcommand{\divS}{\operatorname{div}_{\! \SurfDomain}\!}

\newcommand{\GradP}{\GradSymbol_{\!\ProjMat}\!}
\newcommand{\DivP}{\operatorname{div}_{\!\ProjMat}\!}

\newcommand{\GradC}{\GradSymbol_{\!C}\!}
\newcommand{\DivC}{\operatorname{div}_{\!C}\!}

\newcommand{\LapSurf}{\Lap_{\SurfDomain}}
\newcommand{\GradSurfH}{\GradSymbol_{\SurfDomain[\meshparam]}}
\newcommand{\DivSurfH}{\GradSurfH\cdot}
\newcommand{\LapSurfH}{\Lap_{\SurfDomain[\meshparam]}}

\newcommand{\GradSurfConv}[1]{\GradSymbol_{#1}}

\newcommand{\GradSurfcoord}[1]{\underline{D}_{#1}}

\newcommand{\gradDef}[1]{\eth_{#1}}
\newcommand{\gradDefMat}[1]{\gradDef{#1}^{\SurfDomain}}
\newcommand{\gradDefLower}[1]{\gradDef{#1}^{b}}

\newcommand{\gradFunc}[1]{\mathbf{D}_{#1}}

\newcommand{\Der}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\partial}
  {\partial_{\scriptscriptstyle{#1}}}
}
\newcommand{\DerT}{\Der_{\Time}\,}
\newcommand{\DerPar}[2]{\frac{\Der #1}{\Der #2}}
\newcommand{\tDerPar}[2]{\tfrac{\Der #1}{\Der #2}}
\newcommand{\DerParT}[1]{\DerPar{#1}{\Time}}
\newcommand{\DerParIL}[2]{{\Der #1}/{\Der #2}}
\newcommand{\DerTot}[2][t]
{
  \ifthenelse{\equal{#2}{}}
  {\frac{d #2}{dt}}
  {\frac{d #2}{d #1}}
}
\newcommand{\Derd}[2][]{
  \ifthenelse{\equal{#1}{}}
  {\Diffsymbol{#2}}
  {\Diffsymbol_{{#1}}{#2}}
}
\newcommand{\Diffsymbol}{\operatorname{d}\!}
\newcommand{\Diff}[2][]{
  \ifthenelse{\equal{#1}{}}
  {\Diffsymbol{#2}}
  {\Diffsymbol{#2}_{{#1}}}
}
\newcommand{\DirDerSymb}{D}
\newcommand{\DirDer}[2][]
{
  \ifthenelse{\equal{#1}{}}
  {\DirDerSymb^{#2}}
  {\DirDerSymb^{#2}_{#1}}
}

\newcommand{\tr}{\operatorname{tr}}

\newcommand{\Graph}[1]{\operatorname{Graph}(#1)}

\newcommand{\BigO}[1]{\ensuremath{\operatorname{\mathcal{O}}\!\left(#1\right)}}
\newcommand{\LittleO}[1]{\ensuremath{\operatorname{\mathpzc{o}}\!\left(#1\right)}}
\newcommand{\Rank}[1]{\ensuremath{\operatorname{rank}\left(#1\right)}}
\newcommand{\Exp}[1]{\ensuremath{\operatorname{e}^{#1}}}
\newcommand{\ExpIL}[1]{\ensuremath{\operatorname{exp}({#1})}}
\newcommand{\REALsymbol}{\mathbb{R}}
\newcommand{\REAL}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\REALsymbol}
  {{\REALsymbol}^{#1}}
}
\newcommand{\EUCLsymbol}{\mathbb E}
\newcommand{\EUCL}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\EUCLsymbol}
  {{\EUCLsymbol}^{#1}}
}
\newcommand{\NATURALsymbol}{\mathbb N}
\newcommand{\NATURAL}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\NATURALsymbol}
  {{\NATURALsymbol}^{#1}}
}

\newcommand{\dist}[2]{\operatorname{dist}(#1,#2)}

\newcommand{\ABS}[2][]
{
  \ifthenelse{\equal{#1}{}}
  {\left| #2 \right|}
  {\left| #2 \right|_{#1}}
}

\newcommand{\ABSSurf}[1]{\ensuremath{\left|#1\right|_{\SurfDomain}}}

\newcommand{\NORM}[2][]
{
  \ifthenelse{\equal{#1}{}}
  {\left\| #2 \right\|}
  {\left\| #2 \right\|_{#1}}
}
\newcommand{\vertiii}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}
\newcommand{\BrNORM}[2][]
{
  \ifthenelse{\equal{#1}{}}
  {\vertiii{#2}}
  {\vertiii{#2}_{#1}}
}

\newcommand{\SCAL}[3][]
{
  \ifthenelse{\equal{#1}{}}
  {\left\langle{#2},{#3}\right\rangle}
  {\left\langle{#2},{#3}\right\rangle_{#1}}
}
\newcommand{\SCALF}[3][]
{
  \ifthenelse{\equal{#1}{}}
  {\left({#2},{#3}\right)}
  {\left({#2},{#3}\right)_{#1}}
}
\newcommand{\CSCALF}[2]{{C}\left(#1,#2\right)}
\newcommand{\BSCALF}[2]{b\left(#1,#2\right)}
\newcommand{\BSCALFH}[2]{b_h\left(#1,#2\right)}
\newcommand{\DSCALF}[2]{d\left(#1,#2\right)}
\newcommand{\scalar}[2]{\prodscal{#1}{#2}}
\newcommand{\scalprod}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\scalprodSurf}[3][]
{
  \ifthenelse{\equal{#1}{}}
  {\left\langle {#2},{#3} \right\rangle_{\scriptscriptstyle\SurfDomain}}
  {\left\langle {#2},{#3} \right\rangle_{{#1}}}
}
\newcommand{\Lie}[2]{\left[#1,#2\right]}
\newcommand{\DET}[1]{\ensuremath{\operatorname{det}(#1)}}
\newcommand{\Trace}[1]{\ensuremath{\operatorname{Tr}(#1)}}
\newcommand{\Inner}[2]{\left({#1}\,,\,{#2}\right)_{\SurfDomain}}
\newcommand{\InnerApprox}[2]{\left({#1}\,,\,{#2}\right)_{\meshparam}}
%_{\SurfDomain[\meshparam]}}

\newcommand{\Origin}{\mathbf{o}} % the origin 
\newcommand{\Point}{\mathbf{P}}
\newcommand{\point}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\mathbf{p}}
  {\mathbf{p}_{#1}}
}
\newcommand{\Qpoint}{\mathbf{Q}}
\newcommand{\qpoint}{\mathbf{q}}
\newcommand{\qvalue}{q}
\newcommand{\rpoint}{\mathbf{r}}
\newcommand{\mpoint}{\mathbf{m}}
\newcommand{\midPoint}{\mathbf{m}}
\newcommand{\lform}[1]{{f}\left(#1\right)}
\newcommand{\Lform}[1]{{L}\left(#1\right)}
\newcommand{\Poly}{\mathcal{P}}
\newcommand{\RT}{\mathcal{RT}}
\newcommand{\Const}{\mathcal{C}}

\newcommand{\Dt}{\Delta\tempo}
\newcommand{\Dx}{\Delta x}

\newcommand{\From}{:}
\newcommand{\To}{\longrightarrow}
\newcommand{\Mapsto}{\longmapsto}
%\newcommand{\Closure}[1]{\overline{#1}}
\newcommand{\Closure}[1]{\operatorname{cl}({#1})}

% Domain 
\newcommand{\Domain}{\Omega}
\newcommand{\Bnd}{\partial \Omega}
\newcommand{\RegionSymb}{R}
\newcommand{\Region}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\RegionSymb}
  {\RegionSymb_{#1}}
}
\newcommand{\PartitionRegion}{\mathcal{R}}
\newcommand{\diam}{\operatorname{diam}}
\newcommand{\diamReg}{\diam\Region}
\newcommand{\IT}{[0,\TimeF]} % time interval
\newcommand{\Interval}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {I}
  {I_{#1}}
}
\newcommand{\tInterval}{\tilde{I}}
\newcommand{\SurfDomainsymb}{\mathcal{S}}
\newcommand{\SurfDomain}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\SurfDomainsymb}
  {{\SurfDomainsymb_{#1}}}
}
\newcommand{\tSurfDomain}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\tilde{\SurfDomainsymb}}
  {\tilde{\SurfDomainsymb}_{#1}}
}
\newcommand{\SurfDomainBndsymb}{\partial\Gamma}
\newcommand{\SurfDomainBnd}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\SurfDomainBndsymb}
  {\SurfDomainBndsymb_{#1}}
}
\newcommand{\ClosedSurfDomain}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\Closedsymb{\SurfDomain}}
  {\Closedsymb{\SurfDomain[#1]}}
}

\newcommand{\curve}{\sigma}
\newcommand{\tcurve}{\tilde{\curve}}
\newcommand{\DerCurve}{{\curve}'}
\newcommand{\tDerCurve}{{\tcurve}'}
\newcommand{\curveparam}{\lambda}
\newcommand{\bcurveparam}{\tau}


\newcommand{\FSMsymbol}{\mathcal{F}}
\newcommand{\BSMsymbol}{\mathcal{B}}
\newcommand{\LSMsymbol}{\mathcal{L}}
\newcommand{\SSMsymbol}{\mathcal{M}}
\newcommand{\FSM}
  {\FSMsymbol}
\newcommand{\BSM}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\BSMsymbol}
  {\BSMsymbol_{#1}}
}
\newcommand{\LSM}
  {\LSMsymbol}
\newcommand{\SSM}
  {\SSMsymbol}
\newcommand{\FreeWaterSurfHat}{\mathcal{S}_{\hat{\FSMsymbol}}}
\newcommand{\FreeWaterSurf}{\mathcal{S}_\FSMsymbol}
\newcommand{\Bottom}{\mathcal{S}_\BSMsymbol}
\newcommand{\Lateral}{\mathcal{S}_\LSMsymbol}
\newcommand{\Surf}{\mathcal{S}}
\newcommand{\BoundSurf}{\SSMsymbol}
\newcommand{\SurfBndsymb}{\partial\Surf}
\newcommand{\SurfBnd}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\SurfBndsymb}
  {\SurfBndsymb_{#1}}
}
\newcommand{\Closedsymb}[1]{\bar{#1}}
\newcommand{\ClosedSurf}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\Closedsymb{\Surf}}
  {\Closedsymb{\Surf[#1]}}
}

% symbol for vectors
%\newcommand{\Vector}[1]{\mathbf{#1}}

\newcommand{\press}{p}
\newcommand{\tpress}{\tilde{\press}}
\newcommand{\grav}{g}
\newcommand{\gravpot}{\zcg}
\newcommand{\vectgrav}{\mathbf{g}}
\newcommand{\Depth}{\eta}
\newcommand{\tension}{\sigma}
\newcommand{\ttension}{\tilde{\tension}}
\newcommand{\densitySymb}{\rho}
\newcommand{\density}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\densitySymb}
  {\densitySymb_{\scriptscriptstyle{#1}}}
}

\newcommand{\eb}{\boldsymbol{e}} %for Cartesian base vector fields

\newcommand{\concSymbol}{\phi}
\newcommand{\CHsol}{\concSymbol}
\newcommand{\CHsolApprox}{\CHsol_{\meshparam}}
\newcommand{\pressApprox}{\press_{\meshparam}}

\newcommand{\dWellSymbol}{W}
\newcommand{\dWell}{\dWellSymbol}
\newcommand{\mobilitySymbol}{m}
\newcommand{\mobility}{\mobilitySymbol}
\newcommand{\Galpha}{{G_{\alpha}}}
\newcommand{\chempotSub}{\mu_{\scriptscriptstyle{CH}}}
\newcommand{\chempot}{\mu}
\newcommand{\chempotApprox}{\mu_{\meshparam}}

\newcommand{\bendingSymb}{\kappa}
\newcommand{\bendStiff}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\bendingSymb}
  {\bendingSymb_{#1}}
}

\newcommand{\Be}[1]{\operatorname{Be(#1)}}

\newcommand{\bendStiffGauss}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\overline{\bendingSymb}}
  {\overline{\bendingSymb}_{#1}}
}



\newcommand{\Reynolds}{\operatorname{Re}}%\operatorname{Re}}

\newcommand{\idvec}[1]{\boldsymbol{e}_{#1}} % ith identity vector e_i
\newcommand{\idvecT}[1]{\boldsymbol{e}_{#1}^T} % identity vector transposed

% Order parameter
\newcommand{\AspRatio}{\epsilon}
\newcommand{\epsCurv}{\AspRatio_{\scriptscriptstyle \First}}
\newcommand{\epsApprox}{\epsCurv}
\newcommand{\interfaceparam}{\AspRatio}


% Maps
\newcommand{\param}{\boldsymbol{X}}

\newcommand{\update}{\boldsymbol{Y}}
\newcommand{\updateApprox}{\update_{\meshparam}}

\newcommand{\MapUsymb}{\param}
\newcommand{\MapU}[1][]
{
  \ifthenelse{\equal{#1}{}}
    {\MapUsymb}
    {\MapUsymb_{#1}}
}
\newcommand{\MapLinsymb}{F}
\newcommand{\MapLin}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\ensuremath{\MapLinsymb}}
  {\ensuremath{\MapLinsymb_{#1}}}
}

\newcommand{\MapVsymb}{\psi}
\newcommand{\MapV}[1][]
{
  \ifthenelse{\equal{#1}{}}
    {\MapVsymb}
    {\MapVsymb_{#1}}
}
\newcommand{\Transsymb}{\Phi}
\newcommand{\Trans}[1][]
{
  \ifthenelse{\equal{#1}{}}
    {\Transsymb} 
    {\Transsymb_{\scriptscriptstyle{#1}}}
}
\newcommand{\InvMapsymb}{\Psi}
\newcommand{\InvMap}[1][]
{
  \ifthenelse{\equal{#1}{}}
    {\InvMapsymb}
    {\InvMapsymb_{\scriptscriptstyle{#1}}}
}

\newcommand{\fsymb}{f}
\newcommand{\scalFun}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\fsymb}
  {\fsymb_{#1}}
}
\newcommand{\tscalFun}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\tilde{\fsymb}}
  {\tilde{\fsymb}_{#1}}
}
\newcommand{\bscalFun}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\bar{\fsymb}}
  {\bar{\fsymb}_{#1}}
}
\newcommand{\gsymb}{g}
\newcommand{\scalFung}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\gsymb}
  {\gsymb_{#1}}
}
\newcommand{\Fsymb}{F}
\newcommand{\FvecFun}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\Fsymb}
  {\Fsymb_{#1}}
}
\newcommand{\tFvecFun}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\tilde{\Fsymb}}
  {\tilde{\Fsymb}_{#1}}
}
\newcommand{\Ffunc}[2][]
{
  \ifthenelse{\equal{#1}{}}
  {\ensuremath{\Fsymb_{#2}}}
  {\ensuremath{\Fsymb^{#1}_{#2}}}
}
\newcommand{\Gsymb}{g}
\newcommand{\Gfun}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\ensuremath{\Gsymb}}
  {\ensuremath{\Gsymb_{{#1}}}}
}
\newcommand{\bGfun}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\ensuremath{\bar{\Gsymb}}}
  {\ensuremath{\bar{\Gsymb}_{{#1}}}}
}
\newcommand{\bGfunApprox}{\bGfun[\meshparam]}
\newcommand{\preimagesymb}{{-1}} %\leftarrow
\newcommand{\preimage}[2]{#1^\preimagesymb(#2)}
\newcommand{\inverse}[1]{#1^{-1}}

\newcommand{\Jac}{\mathbf{J}}
\newcommand{\Hess}{\mathbf{H}}
\newcommand{\PrincipalK}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {k}
  {k_{#1}}
}

\newcommand{\vecsymb}{u}
\newcommand{\vecFun}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\Vector{\vecsymb}}
  {\vecsymb^{#1}}
}
\newcommand{\tvecFun}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\tilde{\vecsymb}}
  {\tilde{\vecsymb}_{#1}}
}

% Vectors
\newcommand{\wwsymb}{w}
\newcommand{\ww}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\mathbf{\wwsymb}}
  {\wwsymb^{#1}}
}
\newcommand{\uusymb}{u}
\newcommand{\uu}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\mathbf{\uusymb}}
  {\uusymb^{#1}}
}
\newcommand{\positVec}{\mathbf{r}}

\newcommand{\VecFieldSymbol}{X}
\newcommand{\VecField}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\VecFieldSymbol}
  {\VecFieldSymbol^{#1}}
}
\newcommand{\VecFieldSymbolC}{Y}
\newcommand{\VecFieldYSymbol}{\boldsymbol{\VecFieldSymbolC}}
\newcommand{\VecFieldY}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\VecFieldYSymbol}
  {\VecFieldYSymbol^{#1}}
}
\newcommand{\VecFieldYC}{\VecFieldSymbolC}


\newcommand{\xvsymb}{x}
\newcommand{\xv}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\mathbf{\xvsymb}}
  {\mathbf{\xvsymb}_{\scriptscriptstyle{#1}}}
}
\newcommand{\xvcomp}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\xvsymb}
  {\xvsymb^{\scriptscriptstyle{#1}}}
}
\newcommand{\xcg}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\xvcomp[1]}
  {\xvcomp[1]_{\scriptscriptstyle{#1}}}
}
\newcommand{\ycg}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\xvcomp[2]}
  {\xvcomp[2]_{\scriptscriptstyle{#1}}}
}
\newcommand{\zcg}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\xvcomp[3]}
  {\xvcomp[3]_{\scriptscriptstyle{#1}}}
}
\newcommand{\gcscomp}{\xcg,\ycg,\zcg}

% reference triangle coordinates
\newcommand{\Reftrianglesymb}{\zeta}
\newcommand{\Refcomp}[1]{\Reftrianglesymb^{#1}}
\newcommand{\Refx}{\Reftrianglesymb^1}
\newcommand{\Refy}{\Reftrianglesymb^2}
\newcommand{\zv}{\mathbf{\Reftrianglesymb}}

\newcommand{\svsymb}{s}
\newcommand{\sv}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\mathbf{\svsymb}}
  {\mathbf{\svsymb}_{\scriptscriptstyle{#1}}}
}
\newcommand{\svcomp}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\svsymb}
  {\svsymb^{\scriptscriptstyle{#1}}}
}
\newcommand{\xcl}[1][]{
  \ifthenelse{\equal{#1}{}}
   {\svcomp[1]}
   {\svcomp[1]_{\scriptscriptstyle{#1}}}
}
\newcommand{\ycl}[1][]{
  \ifthenelse{\equal{#1}{}}
   {\svcomp[2]}
   {\svcomp[2]_{\scriptscriptstyle{#1}}}
}
\newcommand{\zcl}[1][]{
  \ifthenelse{\equal{#1}{}}
   {\svcomp[3]}
   {\svcomp[3]_{\scriptscriptstyle{#1}}}
}
\newcommand{\lcscomp}{\xcl,\ycl,\zcl}

% Tangent Plane
\newcommand{\ProjSymb}{\operatorname{\pi}}
\newcommand{\ProjFun}[2][]{
  \ifthenelse{\equal{#1}{}}
  {\ProjSymb\left(#2\right)}
  {\ProjSymb_{\scriptscriptstyle{#1}}\left(#2\right)}
}
\newcommand{\Prm}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\operatorname{pr}}
  {\operatorname{pr}_{\scriptscriptstyle{#1}}}
}
\newcommand{\TanPlane}[2][]
{
  \ifthenelse{\equal{#1}{}}
  {T_{\scriptscriptstyle{\point}}#2}
  {T_{\scriptscriptstyle{#1}}#2}
}
\newcommand{\Tbundle}[1]{\operatorname{T}{#1}}
\newcommand{\Vbundle}{\operatorname{E}} 

%  Subsets
\newcommand{\SubsetSymbol}{\mathcal{U}}
\renewcommand{\Subset}{\SubsetSymbol}
%
\newcommand{\SubsetU}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {{U}}
  {{U}_{#1}}
}
\newcommand{\SubsetV}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {{V}}
  {{V}_{#1}}
}
\newcommand{\SubsetW}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {{W}}
  {{W}_{#1}}
}
\newcommand{\NeighSymbol}{\mathcal{N}}
\newcommand{\Neigh}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\NeighSymbol_{\point}}
  {\NeighSymbol_{#1}}
}
\newcommand{\NeighSurf}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\SubsetSymbol_{\point}}
  {\SubsetSymbol_{#1}}
}
% normal vector to the surface
\newcommand{\NormSymb}{\nu}
\newcommand{\normalvec}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\boldsymbol{\NormSymb}}
  {\NormSymb_{#1}}
}\newcommand{\normalvecApprox}{\NormSymb_{\meshparam}}
\newcommand{\normalSurf}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\NormSymb}
  {\NormSymb(#1)}
}
\newcommand{\normalInterp}[1][]
{
  \ifthenelse{\equal{#1}{}}
   {\tilde{\NormSymb}}
   {\tilde{\NormSymb}_{\scriptscriptstyle{#1}}}
}

% normal vector to the cell edge
\newcommand{\normalEdge}{\mathbf{\nu}} 
\newcommand{\basisCC}{t}
\newcommand{\basisGC}{e}
\newcommand{\vecBaseGC}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\mathbf{\basisGC}}
  {\mathbf{\basisGC}_{#1}}
}
\newcommand{\vecBasePhys}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\mathbf{\basisGC}}
  {\mathbf{\basisGC}_{#1}}
}

% Reference vectors
\newcommand{\vecBaseCCcv}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\mathbf{\basisCC}}
  {\mathbf{\basisCC}_{#1}}
}
\newcommand{\tangential}{\vecBaseCCcv[1],\vecBaseCCcv[2],\vecBaseCCcv[3]}

\newcommand{\tvecBaseCCcv}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\tilde{\mathbf{\basisCC}}}
  {\tilde{\mathbf{\basisCC}}_{#1}}
}
\newcommand{\hvecBaseCCcv}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\hat{\mathbf{\basisCC}}}
  {\hat{\mathbf{\basisCC}}_{#1}}
}
\newcommand{\vecBaseCCctrv}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\mathbf{\basisCC}}
  {\mathbf{\basisCC}^{#1}}
}

\newcommand{\metricsymbol}{g}
\newcommand{\metrTensCv}[1]{\metricsymbol_{\mbox{\tiny{#1}}}}
\newcommand{\hatmetrTensCv}[1]{\hat{\metricsymbol}_{\mbox{\tiny{#1}}}}
\newcommand{\metrTensCtrv}[1]{\metricsymbol^{#1}}
\newcommand{\metrcoefsymbol}{h}
\newcommand{\metrcoef}[1]{\metrcoefsymbol_{\mbox{\tiny{(#1)}}}}
\newcommand{\metrcoefDef}[1]{
  \sqrt{
    \left(\frac{\Der\xcg}{\Der\sv_{#1}}\right)^2
   +\left(\frac{\Der\ycg}{\Der\sv_{#1}}\right)^2
   +\left(\frac{\Der\zcg}{\Der\sv_{#1}}\right)^2}
 }
\newcommand{\defVecBaseCCcv}[1]
{
  \left(
    \dfrac{\Der\xcg[]}{\Der\svcomp[#1]},
    \dfrac{\Der\ycg[]}{\Der\svcomp[#1]}, 
    \dfrac{\Der\zcg[]}{\Der\svcomp[#1]} 
  \right)
}


\newcommand{\first}[1]{
  \IfEqCase{#1}{
    {1}{\operatorname{E}}
    {2}{\operatorname{F}}
    {3}{\operatorname{G}}
  }
  [\PackageError{first}{Undefined option to first: #1}{}]%
}
\newcommand{\SecondFormSymbol}{\ensuremath{\operatorname{II}}}
\newcommand{\SecondForm}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\SecondFormSymbol_{\point}}
  {\SecondFormSymbol_{#1}}
}
\newcommand{\second}[1]{
  \IfEqCase{#1}{
    {1}{\operatorname{e}}
    {2}{\operatorname{f}}
    {3}{\operatorname{g}}
  }
  [\PackageError{first}{Undefined option to first: #1}{}]
}
\newcommand{\WeigSymbol}{\mathcal{W}}
\newcommand{\Weig}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\WeigSymbol}
  {\WeigSymbol_{#1}}
}
\newcommand{\ChristSymb}[2]{\Gamma_{#1}^{#2}}

\newcommand{\face}{{\sigma}}
\newcommand{\parvar}{\sigma}

\newcommand{\DivEins}[2][]{
  {\dfrac{\Der {#2}}{\Der #1}}
}

% Velocity vectors
\newcommand{\velSymbol}{\boldsymbol{u}}
\newcommand{\vectvel}[1][]
{
   \ifthenelse{\equal{#1}{}}
   {\mathbf{\velSymbol}}
   {\mathbf{\velSymbol}(#1)}
}
\newcommand{\velVSymbol}{\boldsymbol{w}}
\newcommand{\vectvelV}[1][]
{
   \ifthenelse{\equal{#1}{}}
   {\mathbf{\velVSymbol}}
   {\mathbf{\velVSymbol}(#1)}
}
\newcommand{\vectvelApprox}[1][]
{
   \ifthenelse{\equal{#1}{}}
   {\mathbf{\velSymbol}_{\meshparam}}
   {\mathbf{\velSymbol}_{\meshparam}(#1)}
}
\newcommand{\redvectvel}{
  \underline{
     \vec{\velSymbol}
     }
}
\newcommand{\velcompContr}[2][i]
{
   \ifthenelse{\equal{#2}{}}
   {\velSymbol^{#1}}
   {\velSymbol^{#1}(#2)}}
\newcommand{\velcompPhys}[2][i]
{
   \ifthenelse{\equal{#2}{}}
   {\velSymbol_{(#1)}}
   {\velSymbol_{(#1)}(#2)}}
\newcommand{\velcomp}{\velcompContr}%{\velcompPhys}


\newcommand{\velSymbolRP}{v}
\newcommand{\velcompContrRP}[2][i]
{
   \ifthenelse{\equal{#2}{}}
   {\velSymbolRP^{#1}}
   {\velSymbolRP^{#1}(#2)}}
\newcommand{\velRP}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\velSymbolRP}
  {\velSymbolRP_{#1}}
}
\newcommand{\velcompRP}{\velRP}        

\newcommand{\velcompApprox}[2][i]
{
   \ifthenelse{\equal{#2}{}}
   {\velSymbol^{#1)}}
   {\velSymbol^{#1}_{(#2)}}
}

% surface cordinates
\newcommand{\coord}{\mathbf{x}}
\newcommand{\coordC}{x}



% Depth average velocity
\newcommand{\VelSymbol}{U}
\newcommand{\vectVel}[1][]
{
   \ifthenelse{\equal{#1}{}}
   {\vec{\VelSymbol}}
   {\vec{\VelSymbol}(#1)}
}
\newcommand{\Velcomp}[2][i]
{
   \ifthenelse{\equal{#2}{}}
   {\VelSymbol^{#1}}
   {\VelSymbol^{#1}(#2)}
}
\newcommand{\VprimoSymbol}{\tilde{u}}
\newcommand{\Vprimo}[1][]
{
   \ifthenelse{\equal{#1}{}}
   {\VprimoSymbol}
   {\VprimoSymbol(#1)}
}
\newcommand{\VprimoComp}[2][i]
{
   \ifthenelse{\equal{#2}{}}
   {\VprimoSymbol^{#1}}
   {\VprimoSymbol^{#1}(#2)}
}
\newcommand{\ttvelSymbol}{\tilde{\Mymathbb{u}}}
\newcommand{\ttvel}[1][]
{
   \ifthenelse{\equal{#1}{}}
   {\mathbf{\ttvelSymbol}}
   {\mathbf{\ttvelSymbol}(#1)}
}
\newcommand{\ttvelComp}[2][i]
{
   \ifthenelse{\equal{#2}{}}
   {\ttvelSymbol^{#1}}
   {\ttvelSymbol^{#1}(#2)}
}

% alpha
\newcommand{\alphaSymbol}{\alpha}
\newcommand{\alphacomp}[1]{\alphaSymbol_{#1}}
\newcommand{\MatAlphaSymbol}{\mathbb{A}}
\newcommand{\MatAlpha}[1][]{%
  \ifthenelse{\equal{#1}{}}
  {\MatAlphaSymbol}
  {\MatAlphaSymbol_{#1}}
}

% Discharge
\newcommand{\QSymbol}{q}
\newcommand{\Qdisch}[1][]
{
   \ifthenelse{\equal{#1}{}}
   {\mathbf{\QSymbol}}
   {\mathbf{\QSymbol}(#1)}
}
\newcommand{\Qcomp}[2][i]
{
   \ifthenelse{\equal{#2}{}}
   {\QSymbol^{#1}}
   {\QSymbol^{#1}(#2)}
}
\newcommand{\Qvect}[1][]
{
   \ifthenelse{\equal{#1}{}}
   {\mathbf{\QSymbol}}
   {\mathbf{\QSymbol}(#1)}
}
% Friction vector
\newcommand{\FricSymbol}{f}
\newcommand{\vectFric}[1][]
{
   \ifthenelse{\equal{#1}{}}
   {\mathbf{\FricSymbol}}
   {\mathbf{\FricSymbol}_{\scriptscriptstyle{#1}}}
}
\newcommand{\Friccomp}[2][i]
{
   \ifthenelse{\equal{#2}{}}
   {\FricSymbol_{#1}}
   {\FricSymbol_{#1}(#2)}}
%
\newcommand{\BFsymbol}{\tau}
\newcommand{\BottomFriction}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\BFsymbol_{b}}
  {\BFsymbol_{b}^{#1}}
}

% Tensors
\newcommand{\ProjMatSymb}{\boldsymbol{P}}
\newcommand{\ProjMat}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\ProjMatSymb}
  {\ProjMatSymb_{#1}}
}
\newcommand{\IDSymbol}{\boldsymbol{I}}
\newcommand{\IDtens}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\IDSymbol}
  {\IDSymbol(#1)}
}
\newcommand{\IDMat}{\IDSymbol}
\newcommand{\Onevect}{\Mymathbb{1}}

\newcommand{\tensSymbol}{\boldsymbol{T}}
\newcommand{\tenscompSymbol}{\tau}
\newcommand{\tens}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\tensSymbol}
  {\tensSymbol(#1)}
}
\newcommand{\tenscomp}[2][ij]
{
  \ifthenelse{\equal{#2}{}}
  {\tenscompSymbol^{#1}}
  {\tenscompSymbol^{#1}(#2)}
}
\newcommand{\tensrow}[2][i]
{
  \ifthenelse{\equal{#2}{}}
  {\tensSymbol^{(#1)}}
  {\tensSymbol^{(#1)}(#2)}
}
% Depth averaged tensor
\newcommand{\TensSymbol}{\mathbf{T}}
\newcommand{\Tens}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\TensSymbol}
  {\TensSymbol_{#1}}
}

\newcommand{\TensCompSymbol}{\TensSymbol}
\newcommand{\TensComp}[2][ij]
{
  \ifthenelse{\equal{#2}{}}
  {\TensCompSymbol^{#1}}
  {\TensCompSymbol^{#1}(#2)}
}

\newcommand{\tensPrimoSymbol}{\tilde{\mathbf{\tau}}}
\newcommand{\tensPrimo}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\tensPrimoSymbol}
  {\tensPrimoSymbol(#1)}
}
\newcommand{\tensPrimoCompSymbol}{\tensPrimoSymbol}
\newcommand{\tensPrimoComp}[2][ij]
{
  \ifthenelse{\equal{#2}{}}
  {\tensPrimoCompSymbol^{#1}}
  {\tensPrimoCompSymbol^{#1}(#2)}
}
% metric coefficients h_i
\newcommand{\MCxl}[1][]{\ifthenelse{\equal{#1}{}}{h_{(1)}}{h_{(1),#1}}} 
\newcommand{\MCyl}[1][]{\ifthenelse{\equal{#1}{}}{h_{(2)}}{h_{(2),#1}}} 
\newcommand{\MCzl}[1][]{\ifthenelse{\equal{#1}{}}{h_{(3)}}{h_{(3),#1}}}
% derivative of z of global coordinates over s1 
\newcommand{\DzgDxl}{\dfrac{\Der\zcg}{\Der\xcl}} 
\newcommand{\DzgDyl}{\dfrac{\Der\zcg}{\Der\ycl}} 
\newcommand{\DzgDzl}{\dfrac{\Der\zcg}{\Der\zcl}}
% derivative of bottom surface over s1
\newcommand{\DbottDxl}{\dfrac{\Der \BSM}{\Der \xcl}} 
\newcommand{\DbottDyl}{\dfrac{\Der \BSM}{\Der \ycl}}
\newcommand{\DbottDzl}{\dfrac{\Der \BSM}{\Der \zcl}}

\newcommand{\MPsymb}{h}
\newcommand{\Lev}{\ell}
\newcommand{\smallestH}[1][]
{
  \ifthenelse{\equal{#1}{}}
    {{l}}
    {{l}_{#1}}
}
\newcommand{\meshparam}[1][]
{
  \ifthenelse{\equal{#1}{}}
    {\MPsymb}
    {\MPsymb_{\scriptscriptstyle{#1}}}
}
\newcommand{\InradiusSymbol}{r}
\newcommand{\Inradius}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\InradiusSymbol}
  {\InradiusSymbol_{\scriptscriptstyle{#1}}}
}
\newcommand{\Tsymb}{\mathcal{T}}
\newcommand{\Triang}[1][]
{
  \ifthenelse{\equal{#1}{}}
    {\Tsymb}
    {\Tsymb_{#1}}
}
\newcommand{\TriangH}[1][]
{
  \ifthenelse{\equal{#1}{}}
    {\Tsymb_{\meshparam}}
    {\Tsymb_{#1}}
}
\renewcommand{\Triang}{\TriangH}%%%
\newcommand{\Edgesymb}{\sigma}
\newcommand{\Edge}[1][]{
  \ifthenelse{\equal{#1}{}}
    {\Edgesymb}
    {\Edgesymb_{#1}}
}
\newcommand{\EdgeH}[1][]{
  \ifthenelse{\equal{#1}{}}
    {\Edgesymb_{\meshparam}}
    {\Edgesymb_{\meshparam,#1}}
}
\newcommand{\NEdge}[1][]{
  \ifthenelse{\equal{#1}{}}
    {N_{\Edgesymb}}
    {N_{\Edgesymb({#1})}}
}
\newcommand{\Cellsymb}{T}
\newcommand{\Cell}[1][]{
  \ifthenelse{\equal{#1}{}}
    {\Cellsymb}
    {\Cellsymb_{#1}}
}
\newcommand{\tCell}[1][]{
  \ifthenelse{\equal{#1}{}}
    {\tilde{\Cellsymb}}
    {\tilde{\Cellsymb}_{#1}}
}
\newcommand{\CellH}[1][]{
  \ifthenelse{\equal{#1}{}}
    {\Cellsymb_{\meshparam}}
    {\Cellsymb_{\meshparam,#1}}
}
\newcommand{\areaSymb}{\mathcal{A}}
\newcommand{\CellArea}[1][]
{
  \ifthenelse{\equal{#1}{}}
    {\areaSymb_{\Cell}}
    {\areaSymb_{#1}}
}
\newcommand{\CellHArea}[1][]
{
  \ifthenelse{\equal{#1}{}}
    {\areaSymb_{\CellH}}
    {\areaSymb_{\meshparam,#1}}
}

\newcommand{\NCell}[1][]{
  \ifthenelse{\equal{#1}{}}
    {N_{\Cellsymb}}
    {N_{\Cellsymb({#1})}}
}
\newcommand{\GeodCurve}{\mathbf{c}}
\newcommand{\lengthSymb}{l}
\newcommand{\interfaceLength}{\lengthSymb}
\newcommand{\edgeLength}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\lengthSymb_{\Edge}}
  {\lengthSymb_{#1}}
}
\newcommand{\arcLength}{\edgeLength} 
\newcommand{\edgeHLength}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\lengthSymb_{\EdgeH}}
  {\lengthSymb_{\meshparam,#1}}
}
\newcommand{\subVolume}[2]{V_{#1}^{#2}}

\newcommand{\Sourcesymb}{\mathbf{S}}
\newcommand{\Source}[1][]
{
  \ifthenelse{\equal{#1}{}}
    {\Sourcesymb}
    {\Sourcesymb_{#1}}
}
\newcommand{\SourceDepth}{S^{\Depth}}
\newcommand{\SourceQ}{\Sourcesymb^{\Qdisch}}
\newcommand{\SourceTermsMC}[1]{S^{\mbox{\tiny{M}}}_{#1}}
\newcommand{\SourceTermsForces}[1]{S^{\mbox{\tiny{F}}}_{#1}}
\newcommand{\SourceEdge}[1][]{
  \ifthenelse{\equal{#1}{}}
    {\Sourcesymb_{ij}}
    {\Sourcesymb_{#1}}
}

\newcommand{\ConservVar}[2]{\mathbf{U}_{#1}^{#2}}
\newcommand{\ConservVarRP}[2]{\mathbf{V}_{#1}^{#2}}
\newcommand{\tConservVar}[2]{\tilde{\mathbf{U}}_{#1}^{#2}}
\newcommand{\Flux}{\underline{\underline{F}}}
\newcommand{\FluxDepth}{\underline{F}^{\Depth}}
\newcommand{\FluxQ}{\underline{\underline{F}}^{\Qdisch}}
\newcommand{\FluxEdgesymb}{\mathbf{F}}
\newcommand{\FluxEdge}[1][]{
  \ifthenelse{\equal{#1}{}}
    {\FluxEdgesymb_{ij}}
    {\FluxEdgesymb_{#1}}
}
\newcommand{\FluxVec}{\mathbf{F}}
\newcommand{\numFlux}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\tilde{\fsymb}}
  {\tilde{\fsymb}_{#1}}
}
\newcommand{\WBflux}{\mathcal{F}}
\newcommand{\tFluxEdge}[1]{\tilde{\mathbf{F}}^{#1}_{ij}}
\newcommand{\FluxFuncX}{\mathbf{F_1}}
\newcommand{\FluxFuncY}{\mathbf{F_2}}
\newcommand{\FluxFuncNormSymbol}{\mathbf{F}}
\newcommand{\FluxFuncNorm}[1][]{
  \ifthenelse{\equal{#1}{}}
    {\FluxFuncNormSymbol^{\normalEdge}}
    {\FluxFuncNormSymbol^{\normalEdge}_{#1}}    
}
\newcommand{\FluxFuncRP}[1]{\mathbf{F}_{#1}}
\newcommand{\JacobianSymbol}{\mathbf{A}}
\newcommand{\Jacobian}[1][]{
  \ifthenelse{\equal{#1}{}}
    {\JacobianSymbol}
    {\JacobianSymbol_{#1}}    
}
\newcommand{\EValSymbol}{\lambda}
\newcommand{\EVal}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\EValSymbol}
  {\EValSymbol_{#1}}
}
\newcommand{\EVecSymbol}{\mathbf{r}}
\newcommand{\EVec}[2][]{
  \ifthenelse{\equal{#1}{}}
  {\EVecSymbol^{(#2)}}
  {\EVecSymbol^{(#2)}_{#1}}
}


\newcommand{\Sect}[1]{S_{#1}}

%Approximation NORMframe
\newcommand{\nodeA}{A}
\newcommand{\nodeB}{B}
\newcommand{\nodeC}{C}
\newcommand{\nodeAfem}{\point[1]}
\newcommand{\nodeBfem}{\point[2]}
\newcommand{\nodeCfem}{\point[3]}
\newcommand{\nodeDfem}{\point[4]}
\newcommand{\midPointEdge}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\midPoint_{\scriptscriptstyle\Edge}}
  {\midPoint_{\scriptscriptstyle\Edge[#1]}}
}
\newcommand{\gpPointEdgeDG}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\point_{\scriptscriptstyle\Edge}}
  {\point_{\scriptscriptstyle\Edge,#1}}
}
\newcommand{\midPointCell}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\midPoint_{\scriptscriptstyle\Cell}}
  {\midPoint_{\scriptscriptstyle\Cell[#1]}}
}
\newcommand{\tangentCurve}[1]{\tau_{#1}}
\newcommand{\tangentCurveApprox}{\tilde{\tau}_{\scriptscriptstyle{\midPointEdge}}}
\newcommand{\normalSurfApprox}{\normalInterp[\midPointEdge]}
\newcommand{\normalEdgeApprox}{\tilde{\normalEdge}_{\scriptscriptstyle{\midPointEdge}}}
\newcommand{\TanPlaneApprox}{\TanPlane[\midPointEdge]{\SurfDomain}}
\newcommand{\metricApproxEdge}{\tilde{\First}_{\midPointEdge}}
\newcommand{\metricApproxCell}{\tilde{\First}_{\midPointCell}}

\newcommand{\Err}{E}%\varepsilon}
\newcommand{\Eoc}{\mbox{eoc}_{\Lev}}

%Energy
\newcommand{\energySymbol}{\mathcal{F}}
\newcommand{\energy}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\energySymbol}
  {\energySymbol_{#1}}
}
\newcommand{\energyPF}{\energy[PF]}
\newcommand{\energyHelfr}{\energy[H]}
\newcommand{\energyGL}{{\energy[GL]}}
\newcommand{\energyKin}{{\energy[K]}}
%
\newcommand{\Lagrangian}{\mathcal{L}}
\newcommand{\DissPotential}{\mathcal{D}}

% Riemann Solvers
\newcommand{\speedRS}[2][]
{
  \ifthenelse{\equal{#2}{}}
  {S_{#2}}
  {S_{#2}^{#1}}
}
% interpolant
\newcommand{\Interpolant}{I_{\meshparam}}

% Spaces
\newcommand{\ContSymbol}{C}
\newcommand{\Cont}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\ContSymbol^{0}}
  {\ContSymbol^{#1}}
}
\newcommand{\Cinf}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\ContSymbol^{\infty}}
  {\ContSymbol^{\infty}(#1)}
}
\newcommand{\SobSymbol}{W}
\newcommand{\HilbSymbol}{H}
\newcommand{\Hilb}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\HilbSymbol^{1}}
  {\SobSymbol^{1}_{#1}}  
}
\newcommand{\Sob}[2][]{
  \ifthenelse{\equal{#1}{}}
  {\HilbSymbol^{#2}}
  {\SobSymbol^{#2,#1}}  
}

\newcommand{\LspaceSymb}{L}
\newcommand{\Lspace}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\LspaceSymb^{2}}
  {\LspaceSymb^{#1}}  
}
\newcommand{\Linfty}{\LspaceSymb^{\infty}}

\newcommand{\TestSpSymbol}{{V}}
\newcommand{\TestSpace}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\TestSpSymbol({\SurfDomain})}
  {\TestSpSymbol_{#1}({\SurfDomain})}
}

\newcommand{\TestSpaceEmbedded}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\TestSpSymbol(\TriangH(\SurfDomain))}
  {\TestSpSymbol_{#1}(\TriangH(\SurfDomain))}
}
\newcommand{\TestSpaceIntrinsic}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\TestSpSymbol(\Triang(\SurfDomain))}
  {\TestSpSymbol_{#1}(\Triang(\SurfDomain))}
}
\newcommand{\TestSpaceChart}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\TestSpSymbol(\Triang(\SubsetU))}
  {\TestSpSymbol_{#1}(\Triang(\SubsetU))}
}
\newcommand{\TestSpaceCell}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\TestSpSymbol_{\meshparam}(\Cell)}
  {\TestSpSymbol_{\meshparam}(\Cell_{#1})}
}

\newcommand{\TestSpaceVol}{\TestSpace[\meshparam]}
\newcommand{\TestSpaceEmbeddedApprox}{\TestSpaceEmbedded[\meshparam]}
\newcommand{\TestSpaceChartApprox}{\TestSpaceChart[\meshparam]}

\newcommand{\TestSpaceApprox}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\TestSpSymbol_{\meshparam}}
  {\TestSpSymbol_{\meshparam}(#1)}
}
\newcommand{\TestSpaceVec}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\mathbf{\TestSpSymbol}_{\meshparam}}
  {\mathbf{\TestSpSymbol}_{\meshparam}(#1)}
}

\newcommand{\TestSpGammaSymbol}{{P}}
\newcommand{\TestSpaceGamma}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\TestSpGammaSymbol_{\meshparam}}
  {\TestSpGammaSymbol_{\meshparam}(#1)}
}

\newcommand{\TestSpCHSymbol}{{W}}
\newcommand{\TestSpaceCH}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\TestSpCHSymbol_{\meshparam}}
  {\TestSpCHSymbol_{\meshparam}(#1)}
}

\newcommand{\TestSpPressSymbol}{Q}
\newcommand{\TestSpacePress}[1][]{
  \ifthenelse{\equal{#1}{}}
  {\TestSpPressSymbol_{\meshparam}}
  {\TestSpPressSymbol_{\meshparam}(#1)}
}


% Polynomial spaces
\newcommand{\PolySymb}{\mathcal{P}}
\newcommand{\PC}[1]{\PolySymb{_{#1}}}
\newcommand{\PONE}{\PolySymb_{1}}
\newcommand{\PTWO}{\PolySymb_{2}}
\newcommand{\PZERO}{\PolySymb_{0}}


%--------------------------------------------------

\newcommand{\GaussCurv}{\mathcal{K}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\meanCurv}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\calH}
  {\calH_{#1}}
}
\newcommand{\hmeanCurv}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\hat{\calH}}
  {\hat{\calH}_{#1}}
}
\newcommand{\meanCurvApprox}{\meanCurv[\meshparam]}
\newcommand{\shapeOp}{\mathcal{B}}
\newcommand{\AngleSymbol}{\theta}
\newcommand{\DevAngle}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\AngleSymbol}
  {\AngleSymbol_{\scriptscriptstyle{#1}}}
}
\newcommand{\relheightSymb}{\pi}
\newcommand{\relheight}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\relheightSymb_{\scriptscriptstyle{\SurfDomain}}}
  {\relheightSymb_{\scriptscriptstyle{#1}}}
}

\newcommand{\boundarySurf}{\SurfBnd}
\newcommand{\conormal}{\mathbf{\mu}}


\newcommand{\SolSymbol}{u}
\newcommand{\Sol}{\SolSymbol}
\newcommand{\AvgSol}{\bar{\SolSymbol}}
\newcommand{\forceSymbol}{f}
\newcommand{\force}{f}
\newcommand{\forceVecSymbol}{\mathbf{F}}
\newcommand{\forceVec}{\forceVecSymbol}
\newcommand{\AdvVel}{\Vector{w}}
\newcommand{\KinCoef}{\gamma}
\newcommand{\DiffCoef}{\epsilon}
\newcommand{\SolnCoef}{\DiffCoef}
\newcommand{\MassCoef}{c}
\newcommand{\StressTensComp}{\sigma}
\newcommand{\StressTens}{\boldsymbol{\StressTensComp}}
\newcommand{\DiffTens}{\mathbb{D}}
\newcommand{\DiffEig}[1][]
{ \ifthenelse{\equal{#1}{}}
  {d}
  {d_{#1}}
}
\newcommand{\DiffEigMax}{\DiffEig^*}
\newcommand{\DiffEigMin}{\DiffEig_*}

\newcommand{\BilinearStiffSymbol}{a}
\newcommand{\BilinearStiff}[3][]
{
  \ifthenelse{\equal{#1}{}}
  {\BilinearStiffSymbol(#2,#3)}    
  {\BilinearStiffSymbol_{#1}(#2,#3)}    
}
\newcommand{\BilinearAdvSymbol}{b}
\newcommand{\BilinearAdv}[3][]
{
  \ifthenelse{\equal{#1}{}}
  {\BilinearAdvSymbol(#2,#3)}    
  {\BilinearAdvSymbol_{#1}(#2,#3)}    
}
\newcommand{\BilinearMassSymbol}{m}
\newcommand{\BilinearMass}[3][]
{
  \ifthenelse{\equal{#1}{}}
  {\BilinearMassSymbol(#2,#3)}    
  {\BilinearMassSymbol_{#1}(#2,#3)}    
}
\newcommand{\BilinearReactSymbol}{c}
\newcommand{\BilinearReact}[3][]
{
  \ifthenelse{\equal{#1}{}}
  {\BilinearReactSymbol(#2,#3)}    
  {\BilinearReactSymbol_{#1}(#2,#3)}    
}
\newcommand{\MassForm}[2]{m(#1,#2)} 
\newcommand{\Bilinear}[2]{a(#1,#2)}

\newcommand{\RhsSymbol}{F}
\newcommand{\Rhs}[1]{\RhsSymbol(#1)}

\newcommand{\TestSymbol}{v}
\newcommand{\Test}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\TestSymbol}  % test function
  {\TestSymbol_{\scriptscriptstyle{#1}}}
}

% approximation
\newcommand{\SolApprox}{\Sol_{\meshparam}}
\newcommand{\coeffSol}[1]{\Sol_{#1}}
\newcommand{\bcoeffSol}[1]{\bar{\Sol}_{#1}}
\newcommand{\AdvVelApprox}{\mathbf{w}_{\meshparam}}
\newcommand{\forceApprox}{\force_{\meshparam}}

\newcommand{\nodalBasis}[1]{\varphi_{\scriptscriptstyle{#1}}}
\newcommand{\exactBasis}[1]{\bar{\nodalBasis{#1}}}
\newcommand{\indecesBas}{\mathcal{I}}
\newcommand{\supportBas}{S}
\newcommand{\nNodes}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {N^{\scriptscriptstyle{dof}}}
  {N^{\scriptscriptstyle{dof}}_{\scriptscriptstyle{#1}}}
}
\newcommand{\ndof}{3}
\newcommand{\nGPedge}{N^{\scriptscriptstyle{gp}}_{\scriptscriptstyle\Edge}}
\newcommand{\nGPcell}{N^{\scriptscriptstyle{gp}}_{\scriptscriptstyle\Cell}}

\newcommand{\TestApprox}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\TestSymbol_{\scriptscriptstyle{\meshparam}}}  % test function
  {\TestSymbol_{\scriptscriptstyle{\meshparam,#1}}}
}
\newcommand{\coeffTest}[1]{\TestSymbol_{#1}}

\newcommand{\bTestApprox}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\bar{\TestSymbol}_{\scriptscriptstyle{\meshparam}}}  % test function
  {\bar{\TestSymbol}_{\scriptscriptstyle{\meshparam,#1}}}
}

\newcommand{\TestZSymbol}{\mathbf{Z}}
\newcommand{\TestZ}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\TestZSymbol}  % test Z function
  {\TestZSymbol_{\scriptscriptstyle{#1}}}
}

\newcommand{\TestZApprox}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\TestZSymbol_{\scriptscriptstyle{\meshparam}}}  % test Z function
  {\TestZSymbol_{\scriptscriptstyle{\meshparam,#1}}}
}

\newcommand{\TestHSymbol}{{h}}%\mathscr
\newcommand{\TestH}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\TestHSymbol}  % test h function
  {\TestHSymbol_{\scriptscriptstyle{#1}}}
}

\newcommand{\TestHApprox}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\TestHSymbol_{\scriptscriptstyle{\meshparam}}}  % test h function
  {\TestHSymbol_{\scriptscriptstyle{\meshparam,#1}}}
}

\newcommand{\TestWSymbol}{w}
\newcommand{\TestW}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\TestWSymbol}  % test w function
  {\TestWSymbol_{\scriptscriptstyle{#1}}}
}

\newcommand{\TestWApprox}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\TestWSymbol_{\scriptscriptstyle{\meshparam}}}  % test w function
  {\TestWSymbol_{\scriptscriptstyle{\meshparam,#1}}}
}
\newcommand{\bTestWApprox}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\bar{\TestWSymbol}_{\scriptscriptstyle{\meshparam}}}  % test w function
  {\bar{\TestWSymbol}_{\scriptscriptstyle{\meshparam,#1}}}
}

\newcommand{\TestCHSymbol}{\psi}
\newcommand{\TestCHApprox}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\TestCHSymbol_{\scriptscriptstyle{\meshparam}}}  % test psi function (CH)
  {\TestCHSymbol_{\scriptscriptstyle{\meshparam,#1}}}
}
\newcommand{\TestCH}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\TestCHSymbol}  % test psi function (CH)
  {\TestCHSymbol_{\scriptscriptstyle{#1}}}
}
\newcommand{\TestCHmuSymbol}{\xi}
\newcommand{\TestCHmuApprox}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\TestCHmuSymbol_{\scriptscriptstyle{\meshparam}}}  % test mu function (CH)
  {\TestCHmuSymbol_{\scriptscriptstyle{\meshparam,#1}}}
}

\newcommand{\TestVecSymbol}{\boldsymbol{v}}
\newcommand{\TestVecApprox}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\TestVecSymbol_{\scriptscriptstyle{\meshparam}}}  % test vec function (NS)
  {\TestVecSymbol_{\scriptscriptstyle{\meshparam,#1}}}
}
\newcommand{\TestPressSymbol}{q}
\newcommand{\TestPress}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\TestPressSymbol}  % test press function (NS)
  {\TestPressSymbol_{\scriptscriptstyle{#1}}}
}
\newcommand{\TestPressApprox}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\TestPressSymbol_{\scriptscriptstyle{\meshparam}}}  % test press function (NS)
  {\TestPressSymbol_{\scriptscriptstyle{\meshparam,#1}}}
}


\newcommand{\BilinearStiffApprox}[2]{\BilinearStiffSymbol_{\meshparam}(#1,#2)}
\newcommand{\BilinearAdvApprox}[2]{\BilinearAdvSymbol_{\meshparam}(#1,#2)}
\newcommand{\BilinearReactApprox}[2]{\BilinearReactSymbol_{\meshparam}(#1,#2)} 
\newcommand{\BilinearMassApprox}[2]{\BilinearMassSymbol_{\meshparam}(#1,#2)}    
\newcommand{\RhsApprox}[1]{\RhsSymbol_{\meshparam}(#1)}


\newcommand{\BilinearApprox}[2]{a_{\meshparam}(#1,#2)}
\newcommand{\tBilinearApprox}[2]{\tilde{a}_{\meshparam}(#1,#2)}
\newcommand{\MassFormApprox}[2]{m_{\meshparam}(#1,#2)} 
\newcommand{\tMassFormApprox}[2]{\tilde{m}_{\meshparam}(#1,#2)}

\newcommand{\tBilinearStiffApprox}[2]
{\tilde{\BilinearStiffSymbol}_{\meshparam}(#1,#2)}
\newcommand{\tBilinearAdvApprox}[2]
{\tilde{\BilinearAdvSymbol}_{\meshparam}(#1,#2)}    
\newcommand{\tBilinearMassApprox}[2]
{\tilde{\BilinearMassSymbol}_{\meshparam}(#1,#2)}    
 

% matrix form
\newcommand{\vectorRhs}{\mathbf{b}}
\newcommand{\vectorSol}{\mathbf{\Sol}}
\newcommand{\matrixStiff}{\mathbf{A}}
\newcommand{\matrixAdv}{\mathbf{B}}
\newcommand{\matrixReact}{\mathbf{C}}
\newcommand{\matrixMass}{\mathbf{M}}
\newcommand{\vectorRhsDG}{\mathbf{R}}

\newcommand{\tvectorRhs}{\tilde{\vectorRhs}}
\newcommand{\tmatrixStiff}{\tilde{\matrixStiff}}
\newcommand{\tmatrixAdv}{\tilde{\matrixAdv}}
\newcommand{\tmatrixMass}{\tilde{\matrixMass}}
\newcommand{\tmatrixReact}{\tilde{\matrixReact}}


% stabilization
\newcommand{\Peclet}[1]{\operatorname{Pe}_{\scriptscriptstyle{#1}}}
\newcommand{\stabCoef}[1]{\delta_{\scriptscriptstyle{#1}}}
\newcommand{\deltaO}{\delta_0}
\newcommand{\deltaI}{\delta_1}

\newcommand{\stabBil}[2]
{\operatorname{s}_{\scriptscriptstyle{\meshparam}}(#1,#2)}
\newcommand{\stabRhs}[1]{\operatorname{s}_{\RhsSymbol_{\meshparam}}(#1)}


\newcommand{\Stab}{\stabBil}

%% ENTROPY-VISCOSITY
\newcommand{\entropySymb}{E}
\newcommand{\entropy}{\entropySymb}
\newcommand{\entropyVec}{\mathbf{\entropySymb}}
\newcommand{\entrFluxSymb}{G}
\newcommand{\entrFlux}{\mathbf{\entrFluxSymb}}

\newcommand{\massLumped}[1]{m_{#1}}
\newcommand{\Cijcoeff}[1]{\mathbf{c}_{#1}}
\newcommand{\artViscSymbol}{d}
\newcommand{\artVisc}[1]{\artViscSymbol_{#1}}

% \newcommand{\viscositySymb}{\eta}
% \newcommand{\viscosity}[1][]
% {
%   \ifthenelse{\equal{#1}{}}
%   {\viscositySymb}
%   {\viscositySymb_{\scriptscriptstyle{#1}}}
% }

\newcommand{\ResidualSymbol}{R}
\newcommand{\Residual}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\ResidualSymbol}
  {\ResidualSymbol_{#1}}
}

\newcommand{\CPoincare}{C_{_{\SurfDomain}}}
\newcommand{\Ricci}{\operatorname{Ric}}
\newcommand{\Riccibound}{R}
\newcommand{\curvature}[1][]
{
  \ifthenelse{\equal{#1}{}}
  {\kappa}
  {\kappa_{#1}}
}
\newcommand{\Eig}{\lambda_1}

\newcommand{\QuadRule}[2][]
{
  \ifthenelse{\equal{#1}{}}
  {Q(#2)}
  {Q_{#1}(#2)}
}     

\newcommand{\strainTens}{\mathbf{d}}


%Ingos stuff:
\newcommand{\mfrak}{\mathfrak{m}}
\newcommand{\wrt}{w.\,r.\,t.}
%\newcommand{\eg}{e.\,g.}
\newcommand{\st}{s.\,t.} 
\newcommand{\ie}{i.\,e.}
\newcommand{\ia}{i.\,a.}
\newcommand{\oeda}{w.\,l.\,o.\,g.}
%\newcommand{\etc}{etc.}
\newcommand{\resp}{resp.}
\newcommand{\cf}{cf.}

\newcommand{\formComma}{\,\text{,}}
\newcommand{\formPeriod}{\,\text{.}}

\newcommand{\xb}{\boldsymbol{x}}

\newcommand{\wb}{\vectvelV}
\newcommand{\ub}{\vectvel}
%\newcommand{\vb}{\boldsymbol{v}} % too similar to \nu
\newcommand{\vb}{\boldsymbol{\upsilon}}

==> nomenclature.tex <==
\renewcommand{\S}{\mathcal{S}}
\renewcommand{\H}{\mathcal{H}}
\newcommand*{\K}{\mathcal{K}}
\newcommand*{\B}{\mathcal{B}}
\newcommand*{\red}[1]{{\color{red}#1}}
\newcommand*{\Id}{\textbf{Id}}
\renewcommand{\div}{\text{div}}
\newcommand*{\Reyn}{\text{Re}}
\newcommand*{\surfupd}{\eth_{\mathbf{W}} }
\newcommand*{\paramUpdate}{W}
\newcommand*{\LScalar}[2]{\left\langle #1,#2 \right\rangle_h}
\newcommand*{\Tr}{\text{Tr}}
\newcommand*{\F}[1]{\mathcal{F}_{#1}}
\newcommand*{\thickness}{h}
\newcommand*{\vel}{\mathbf{u}}
\newcommand*{\Diss}{\mathcal{D}}
\newcommand*{\R}{\mathbb{R}}
\newcommand*{\viscosity}{\eta}
